Temporal Verification with Answer-Effect Modification

Type-and-effect systems are a widely-used approach to program verification, verifying the result of a computation using types, and the behavior using effects. This paper extends an effect system for verifying temporal, value-dependent properties on event sequences yielded by programs to the delimited control operators shift0/reset0. While these delimited control operators enable useful and powerful programming techniques, they hinder reasoning about the behavior of programs because of their ability to suspend, resume, discard, and duplicate delimited continuations. This problem is more serious in effect systems for temporal properties because these systems must be capable of identifying what event sequences are yielded by captured continuations. Our key observation for achieving effective reasoning in the presence of the delimited control operators is that their use modifies answer effects, which are temporal effects of the continuations. Based on this observation, we extend an effect system for temporal verification to accommodate answer-effect modification. Allowing answer-effect modification enables easily reasoning about traces that captured continuations yield. Another novel feature of our effect system is the support for dependently-typed continuations, which allows us to reason about programs more precisely. We prove soundness of the effect system for finite event sequences via type safety and that for infinite event sequences using a logical relation.

==> defn/fixpoint_semantics.tex <==
\section{Semantics of First-Order Fixpoint Logic}
\label{sec:semlogic}

\par We define the predicate sorts $\esort$ and the partially ordered set $(\fpdom_{\sort}, \sqsubseteq_{\sort})$ and $(\fpdom_{\esort}, \sqsubseteq_{\esort})$ inductively by:
\begin{align*}
  \text{(predicate sorts)} \;
  \esort &::= \propos \mid \seq{\sort} \to \propos
\end{align*}
\par \begin{minipage}{0.48\hsize}
  \begin{align*}
    \fpdom_{\propos} &\defeq \{\top, \bot\} \\
    \fpdom_{\mathbb{Z}} &\defeq \mathbb{Z} \\
    \fpdom_\finiteseq &\defeq \finiteseq \\
    \fpdom_\infiniteseq &\defeq \infiniteseq
  \end{align*}
\end{minipage}
\begin{minipage}{0.48\hsize}
  \begin{align*}
    \sqsubseteq_\propos &\defeq \{(\top, \top), (\bot, \top), (\bot, \bot)\} \\
    \sqsubseteq_{\mathbb{Z}} &\defeq \{(n, n) \mid n \in \mathbb{Z}\} \\
    \sqsubseteq_\finiteseq &\defeq \{(\varpi, \varpi) \mid \varpi \in \finiteseq\} \\
    \sqsubseteq_\infiniteseq &\defeq \{(\pi, \pi) \mid \pi \in \infiniteseq\}
  \end{align*}
\end{minipage}
\begin{align*}
    \fpdom_{\psort} &\defeq
        \{f \in \fpdom_{\psort} \mid
            \allin{\seq{d}_1, \seq{d}_2}{\fpdom_{\seq{\sort}}}{\seq{d}_1 \sqsubseteq_{\seq{\sort}} \seq{d}_2 \Rightarrow f(\seq{d}_1) \sqsubseteq_\propos f(\seq{d}_2)}
        \} \\
    \sqsubseteq_{\psort} &\defeq \{(f, g) \mid
        \all
            {\seq{d} \in \fpdom_{\seq{\sort}}}
            {f(\seq{d}) \sqsubseteq_\propos g(\seq{d})}
    \}
\end{align*}

and, we define conjunction and disjunction of $f, g \in \fpdom_{\psort}$ as follows:
\begin{align*}
    f \sqcap_{\psort} g &\defeq \lamin{\seq{d}}{\fpdom_{\psort}}{f(\seq{d}) \land g(\seq{d})} \\
    f \sqcup_{\psort} g &\defeq \lamin{\seq{d}}{\fpdom_{\psort}}{f(\seq{d}) \lor g(\seq{d})}
\end{align*}

\par Note that $(\fpdom_{\psort}, \sqsubseteq_{\psort})$ forms a complete lattice (See Theorem~\ref{thm:lattice}).
The least and greatest elements of $\fpdom_{\psort}$ are $\lam{\seq{x}}{\bot}$ and $\lam{\seq{x}}{\top}$ respectively.

\par We now define the formal semantics of the first-order fixpoint logic as Fig~\ref{fig:logicsem}.
$\sortsof{A}$ and $\sortsof{f}$ are the sorts sequence of arguments of $A$ and $f$ respectively.

\begin{figure}[H]
    \fbox{\begin{minipage}{\hsize}\vspace{-1em}
        \begin{align*}
            \semFL{\theta}{\top} \\
            \notSemFL{\theta}{\bot} \\
            \semFL{\theta}{\lnot\phi} &\iff \notSemFL{\theta}{\phi} \\
            \semFL{\theta}{\phi_1 \land \phi_2} &\iff \semFL{\theta}{\phi_1} \ \text{and} \ \semFL{\theta}{\phi_2} \\
            \semFL{\theta}{\phi_1 \lor \phi_2} &\iff \semFL{\theta}{\phi_1} \ \text{or} \ \semFL{\theta}{\phi_2} \\
            \semFL{\theta}{\all{x\colon \sort}{\phi}} &\iff \text{for all $d \in \fpdom_\sort$,} \ \semFL{[x\mapsto d]\theta}{\phi} \\
            \semFL{\theta}{\exi{x\colon \sort}{\phi}} &\iff \text{for some $d \in \fpdom_\sort$,} \ \semFL{[x\mapsto d]\theta}{\phi} \\
            \semFL{\theta}{A(\seq{t})} &\iff
                \denote{\seq{t}}_\theta \in \fpdom_{\sortsof{A}} \ \ \text{and} \ 
                \models \denote{A}(\denote{\seq{t}}_\theta) \\
            \semFL{\theta}{X(\seq{t}\colon\seq{\sort})} &\iff
                \denote{\seq{t}}_\theta \in \fpdom_{\seq{\sort}} \ \text{and} \ 
                \text{for all predicates $p$, } \models p(\seq{t}) \\
            \semFL{\theta}{(\lfp{\seq{x}\colon \seq{\sort}}{\phi})(\seq{t})} &\iff
                \semFL
                    {\theta}
                    {\mathit{lfp}^{\psort}(\lam{X}{\lam{\seq{x}}{\phi}})(\seq{t})} \\
            \semFL{\theta}{(\gfp{\seq{x}\colon \seq{\sort}}{\phi})(\seq{t})} &\iff
                \semFL
                    {\theta}
                    {\mathit{gfp}^{\psort}(\lam{X}{\lam{\seq{x}}{\phi}})(\seq{t})} \\
            \denote{x\colon \sort}_\theta &\defeq \theta(x) \in \fpdom_\sort \\
            \denote{f(\seq{t})}_\theta &\defeq \denote{f}(\denote{\seq{t}}_\theta) \in \fpdom_\sort \eqnote{where $\seq{t} \in \fpdom_{\sortsof{f}}$}
        \end{align*}
    \end{minipage}}
    \caption{Semantics of Fixpoint logic formula}
    \label{fig:logicsem}
\end{figure}

\par Here, the least/greatest fixpoint operators$\mathit{lfp}^{\psort}$ and $\mathit{gfp}^{\psort}$ are defined by:
\begin{align*}
    \mathit{lfp}^{\psort}(F) &\defeq {\textstyle \bigsqcap}_{\psort}
        \set{\chi \in \fpdom_{\psort}}{F(\chi) \sqsubseteq_{\psort} \chi} \\
    \mathit{gfp}^{\psort}(F) &\defeq {\textstyle \bigsqcup}_{\psort}
        \set{\chi \in \fpdom_{\psort}}{\chi \sqsubseteq_{\psort} F(\chi)}
\end{align*}

$\bigsqcap_{\psort}$ and $\bigsqcup_{\psort}$
denote respectively the least upper bound and the greatest lower bound with respect to
$\sqsubseteq_{\psort}$.

\begin{theorem}
    \label{thm:lattice}
    $(\fpdom_{\psort}, \sqsubseteq_{\psort})$ forms a complete lattice.
\end{theorem}
\begin{proof}
    \par For any subset of $\fpdom_{\psort}$, $\{p_0, p_1, \cdots p_i\}$, these hold.
    \begin{align*}
        (\lamin{\seq{d}}{\fpdom_{\psort}}{\cumland{j=0}{i}{p_j(\seq{d})}}) \sqsubseteq_{\psort} p_k \\
        p_k \sqsubseteq_{\psort} (\lamin{\seq{d}}{\fpdom_{\psort}}{\cumlor{j=0}{i}{p_j(\seq{d})}})
    \end{align*}
    \par So, this has the least element
    $\lamin{\seq{d}}{\fpdom_{\psort}}{\cumland{k=0}{n}{p_k(\seq{d})}}$ and
    the greatest element
    $\lamin{\seq{d}}{\fpdom_{\psort}}{\cumlor{k=0}{n}{p_k(\seq{d})}}$.
\end{proof}

\begin{theorem}[Continuous]
    For any function $F = \lamin{\chi}{\fpdom_{\psort}}{\lamin{\seq{x}}{\fpdom_{\seq{\sort}}}{\psi}}$
    and any predicate set $S = \{p_0, p_1, \cdots, p_i\}$.
    \begin{align*}
        f({\textstyle \bigsqcup}_{\psort} S) = {\textstyle \bigsqcup}_{\psort}f(S)
    \end{align*}
    where $\psi$ is in negation normal form.
\end{theorem}
\begin{proof}
    By theorem~\ref{thm:lattice}, we get follows:
    \begin{align*}
        f({\textstyle \bigsqcup}_{\psort} S) &= \lam{\seq{x}}
            {[\lam{\seq{y}}{\cumlor{k=0}{i}{p_k(\seq{y})}}/X]\psi} \\
        {\textstyle \bigsqcup}_{\psort} f(S) &= \lam{\seq{x}}
            {\cumlor{k=0}{i}{[p_k/X]\psi}}
    \end{align*}
    So, we show $[\lam{\seq{y}}{\cumlor{k=0}{i}{p_k(\seq{y})}}/X]\psi = \cumlor{k=0}{i}{[p_k/X]\psi}$ by the induction on structure of $\psi$.
    \begin{itemize}
        \item Case $X \notin \fpv{\psi}$. It is obvious.
        \item Case $\psi = \psi_1 \lor \psi_2$.
            By I.H. we have
            \begin{itemize}
                \item $[\lam{\seq{y}}{\cumlor{k=0}{i}{p_k(\seq{y})}}/X]\psi_1 = \cumlor{k=0}{i}{[p_k/X]\psi_1}$
                \item $[\lam{\seq{y}}{\cumlor{k=0}{i}{p_k(\seq{y})}}/X]\psi_2 = \cumlor{k=0}{i}{[p_k/X]\psi_2}$
            \end{itemize}
            So
            \begin{align*}
                [\lam{\seq{y}}{\cumlor{k=0}{i}{p_k(\seq{y})}}/X]\psi &= [\lam{\seq{y}}{\cumlor{k=0}{i}{p_k(\seq{y})}}/X](\psi_1 \lor \psi_2) \\
                &= (\cumlor{k=0}{i}{[p_k/X]\psi_1}) \lor (\cumlor{k=0}{i}{[p_k/X]\psi_2}) \\
                &= \cumlor{k=0}{i}{[p_k/X](\psi_1 \lor \psi_2)}
                = \cumlor{k=0}{i}{[p_k/X]\psi}
            \end{align*}
        \item Case $\psi = \psi_1 \land \psi_2$.
            By I.H. we have
            \begin{itemize}
                \item $[\lam{\seq{y}}{\cumlor{k=0}{i}{p_k(\seq{y})}}/X]\psi_1 = \cumlor{k=0}{i}{[p_k/X]\psi_1}$
                \item $[\lam{\seq{y}}{\cumlor{k=0}{i}{p_k(\seq{y})}}/X]\psi_2 = \cumlor{k=0}{i}{[p_k/X]\psi_2}$
            \end{itemize}
            So
            \begin{align*}
                [\lam{\seq{y}}{\cumlor{k=0}{i}{p_k(\seq{y})}}/X]\psi &= [\lam{\seq{y}}{\cumlor{k=0}{i}{p_k(\seq{y})}}/X](\psi_1 \land \psi_2) \\
                &= (\cumlor{k=0}{i}{[p_k/X]\psi_1}) \land (\cumlor{k=0}{i}{[p_k/X]\psi_2}) \\
                &= \cumlor{k=0}{i}{[p_k/X](\psi_1 \land \psi_2)}
                = \cumlor{k=0}{i}{[p_k/X]\psi}
            \end{align*}
        \item Case $\psi = \all{x}{\psi'}$.
            By I.H. we have
            \begin{itemize}
                \item $[\lam{\seq{y}}{\cumlor{k=0}{i}{p_k(\seq{y})}}/X]\psi' = \cumlor{k=0}{i}{[p_k/X]\psi'}$
            \end{itemize}
            So
            \begin{align*}
                [\lam{\seq{y}}{\cumlor{k=0}{i}{p_k(\seq{y})}}/X]\psi
                    &= \all{x}{[\lam{\seq{y}}{\cumlor{k=0}{i}{p_k(\seq{y})}}/X]\psi'} \\
                    = \all{x}{\cumlor{k=0}{i}{[p_k/X]\psi'}}
                    &= \cumlor{k=0}{i}{[p_k/X]\psi}
            \end{align*}
        \item Case $\psi = \exi{x}{\psi'}$.
            By I.H. we have
            \begin{itemize}
                \item $[\lam{\seq{y}}{\cumlor{k=0}{i}{p_k(\seq{y})}}/X]\psi' = \cumlor{k=0}{i}{[p_k/X]\psi'}$
            \end{itemize}
            So
            \begin{align*}
                [\lam{\seq{y}}{\cumlor{k=0}{i}{p_k(\seq{y})}}/X]\psi
                    &= \exi{x}{[\lam{\seq{y}}{\cumlor{k=0}{i}{p_k(\seq{y})}}/X]\psi'} \\
                    &= \exi{x}{\cumlor{k=0}{i}{[p_k/X]\psi'}}
                    = \cumlor{k=0}{i}{[p_k/X]\psi}
            \end{align*}
        \item Case $\psi = X(\seq{t})$.
            \begin{align*}
                [\lam{\seq{y}}{\cumlor{k=0}{i}{p_k(\seq{y})}}/X]\psi &= (\lam{\seq{y}}{\cumlor{k=0}{i}{p_k(\seq{y})}})(\seq{t})
                = \cumlor{k=0}{i}{p_k(\seq{t})} \\
                &= \cumlor{k=0}{i}{[p_k/X]X(\seq{t})}
                = \cumlor{k=0}{i}{[p_k/X]\psi}
            \end{align*}
    \end{itemize}
\end{proof}

\begin{theorem}[Cocontinuous]
    For any function $F = \lamin{\chi}{\fpdom_{\psort}}{\lamin{\seq{x}}{\fpdom_{\seq{\esort}}}{\psi}}$
    and any predicate set $S = \{p_0, p_1, \cdots, p_i\}$.
    \begin{align*}
        f({\textstyle \bigsqcap}_{\psort} S) = {\textstyle \bigsqcap}_{\psort}f(S)
    \end{align*}
    where $\psi$ is in negation normal form.
\end{theorem}
\begin{proof}
    By theorem~\ref{thm:lattice}, we get follows
    \begin{align*}
        f({\textstyle \bigsqcap}_{\psort} S) &= \lam{\seq{x}}
            {[\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}}/X]\psi} \\
        {\textstyle \bigsqcap}_{\psort} f(S) &= \lam{\seq{x}}
            {\cumland{k=0}{i}{[p_k/X]\psi}}
    \end{align*}
    So, we show $[\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}}/X]\psi = \cumland{k=0}{i}{[p_k/X]\psi}$ by the induction of structure of $\psi$.
    \begin{itemize}
        \item Case $X \notin \fpv{\psi}$. It is obvious.
        \item Case $\psi = \psi_1 \lor \psi_2$.
            By I.H. we have
            \begin{itemize}
                \item $[\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}}/X]\psi_1 = \cumland{k=0}{i}{[p_k/X]\psi_1}$
                \item $[\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}}/X]\psi_2 = \cumland{k=0}{i}{[p_k/X]\psi_2}$
            \end{itemize}
            So
            \begin{align*}
                [\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}}/X]\psi
                    &= [\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}}/X](\psi_1 \lor \psi_2) \\
                    &= ([\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}}/X]\psi_1) \lor ([\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}}/X]\psi_2) \\
                    &= (\cumland{k=0}{i}{[p_k/X]\psi_1}) \lor (\cumland{k=0}{i}{p_k/X}\psi_2) \\
                    &= \cumland{k=0}{i}{[p_k/X](\psi_1 \lor \psi_2)}
                    = \cumland{k=0}{i}{[p_k/X]\psi}
            \end{align*}
        \item Case $\psi = \psi_1 \land \psi_2$.
            By I.H. we have
            \begin{itemize}
                \item $[\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}}/X]\psi_1 = \cumland{k=0}{i}{[p_k/X]\psi_1}$
                \item $[\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}}/X]\psi_2 = \cumland{k=0}{i}{[p_k/X]\psi_2}$
            \end{itemize}
            So
            \begin{align*}
                [\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}}/X]\psi
                    &= [\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}}/X](\psi_1 \land \psi_2) \\
                    &= ([\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}}/X]\psi_1) \land ([\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}}/X]\psi_2) \\
                    &= (\cumland{k=0}{i}{[p_k/X]\psi_1}) \land (\cumland{k=0}{i}{p_k/X}\psi_2) \\
                    &= \cumland{k=0}{i}{[p_k/X](\psi_1 \land \psi_2)}
                    = \cumland{k=0}{i}{[p_k/X]\psi}
            \end{align*}
        \item Case $\psi = \all{x}{\psi'}$.
            By I.H. we have
            \begin{itemize}
                \item $[\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}}/X]\psi' = \cumland{k=0}{i}{[p_k/X]\psi'}$
            \end{itemize}
            So
            \begin{align*}
                [\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}}/X]\psi
                    &= \all{x}{[\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{x})}}/X]\psi'} \\
                    &= \all{x}{\cumland{k=0}{i}{[p_k/X]\psi'}}
                    = \cumland{k=0}{i}{[p_k/X]\psi}
            \end{align*}
        \item Case $\psi = \exi{x}{\psi'}$
            By I.H. we have
            \begin{itemize}
                \item $[\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}}/X]\psi' = \cumland{k=0}{i}{[p_k/X]\psi'}$
            \end{itemize}
            So
            \begin{align*}
                [\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}}/X]\psi
                    &= \exi{x}{[\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}}/X]\psi'} \\
                    &= \exi{x}{\cumland{k=0}{i}{[p_k/X]\psi'}}
                    = \cumland{k=0}{i}{[p_k/X]\psi}
            \end{align*}
        \item Case $\psi = X(\seq{t})$
            \begin{align*}
                [\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}}/X]\psi
                    &= [\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}}/X]X(\seq{t}) \\
                    &= (\lam{\seq{y}}{\cumland{k=0}{i}{p_k(\seq{y})}})(\seq{t})
                    = \cumland{k=0}{i}{p_k(\seq{t})} \\
                    &= \cumland{k=0}{i}{[p_k/X]X(\seq{t})}
                    = \cumland{k=0}{i}{[p_k/X]\psi}
            \end{align*}
    \end{itemize}
\end{proof}


